GDRNPP: A Geometry-guided and Fully Learning-based Object Pose Estimator

6D pose estimation of rigid objects is a long-standing and challenging task in computer vision. Recently, the emergence of deep learning reveals the potential of Convolutional Neural Networks (CNNs) to predict reliable 6D poses. Given that direct pose regression networks currently exhibit suboptimal performance, most methods still resort to traditional techniques to varying degrees. For example, top-performing methods often adopt an indirect strategy by first establishing 2D-3D or 3D-3D correspondences followed by applying the RANSAC-based PnP or Kabsch algorithms, and further employing ICP for refinement. Despite the performance enhancement, the integration of traditional techniques makes the networks time-consuming and not end-to-end trainable. Orthogonal to them, this paper introduces a fully learning-based object pose estimator. In this work, we first perform an in-depth investigation of both direct and indirect methods and propose a simple yet effective Geometry-guided Direct Regression Network (GDRN) to learn the 6D pose from monocular images in an end-to-end manner. Afterwards, we introduce a geometry-guided pose refinement module, enhancing pose accuracy when extra depth data is available. Guided by the predicted coordinate map, we build an end-to-end differentiable architecture that establishes robust and accurate 3D-3D correspondences between the observed and rendered RGB-D images to refine the pose. Our enhanced pose estimation pipeline GDRNPP (GDRN Plus Plus) conquered the leaderboard of the BOP Challenge for two consecutive years, becoming the first to surpass all prior methods that relied on traditional techniques in both accuracy and speed. The code and models are available at https://github.com/shanice-l/gdrnpp_bop2022.

==> figs/ablation_regions.tex <==
% \begin{figure}[t]
%     \begin{center}
%     \includegraphics[width=0.96\linewidth]{figs/ablation_regions_v4.png}
%     \end{center}
%     \vspace{-4mm}
%     \caption{
    % \label{fig:ablate_region}
%         {\bf Ablation on the Number of Regions in $M_\text{SRA}$ on LM.}
%         Although the performance is already good without the guidance of $M_{\text{SRA}}$,
%         it can be improved given more regions as attention.
%         We use $M_{\text{SRA}}$ with 64 regions for accuracy-memory tradeoff.
%     }
%
% \end{figure}


% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.4\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/ablation_regions_v4_a.pdf}\vspace{-2mm}
%         \caption{}
%         \label{fig:ablate_region_a}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.4\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/ablation_regions_v4_b.pdf}\vspace{-2mm}
%         \caption{}
%         \label{fig:ablate_region_b}
%     \end{subfigure}
%     \vspace{-2mm}
%     \caption{
%         \label{fig:ablate_region}
%             {\bf Ablation study for $M_\text{SRA}$ on LM.}
%             Although the performance is already good without the guidance of $M_{\text{SRA}}$,
%             it can be improved given more regions as attention.
%             We use $M_{\text{SRA}}$ with 64 regions for accuracy-memory tradeoff.
%         }
% \end{figure}


==> figs/lm_qualitative.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.95\linewidth]{figs/lm_qualitative_compressed.pdf}
    \end{center}
    \vspace{-4mm}
    \caption{
        \label{fig:lm_qualitative}
        {\bf Qualitative Results on LM~\cite{Hinterstoisser2012}.}
        We visualize the 6D pose by overlaying the image with the corresponding transformed 3D bounding box.
        We demonstrate in \emph{Blue} and \emph{Green} the ground-truth pose and the predicted pose, respectively.
    }
\end{figure*}


==> figs/lmo_qualitative.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.95\linewidth]{figs/lmo_qualitative_compressed.pdf}
    \end{center}
    \vspace{-4mm}
    \caption{
        \label{fig:lmo_qualitative}
        {\bf Qualitative Results on LM-O~\cite{Brachmann2014Learning6O}.}
        For each image, we visualize the 6D poses by rendering the 3D models and overlaying the contours on the right.
        We demonstrate in \emph{Blue} and \emph{Green} the ground-truth pose and the predicted pose, respectively.
    }
\end{figure*}


==> figs/ycbv_qualitative.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.95\linewidth]{figs/ycbv_qualitative_compressed.pdf}
    \end{center}
    \vspace{-4mm}
    \caption{
        \label{fig:ycbv_qualitative}
        {\bf Qualitative Results on YCB-V~\cite{xiang2017posecnn}.}
        For each image, we visualize the 6D poses by rendering the 3D models and overlaying the contours on the right.
        We demonstrate in \emph{Blue} and \emph{Green} the ground-truth pose and the predicted pose, respectively.
    }
\end{figure*}


==> gdrn_tables/bop_det_model.tex <==
\begin{table*}[htbp]
    \centering
\caption{
{\bf Effect of the detector.}
We report the Average Recall (\%) of the BOP metric.
The models leverage real-world data for training on T-LESS, TUD-L and YCB-V datasets.
}    
\tablestyle{8pt}{1.2}
\small
\begin{tabular}{l | cc |ccccccc | c}
        % \shline 
        Method & detector & Modality
        & LM-O & T-LESS & TUD-L & IC-BIN & ITODD & HB & YCB-V & Avg % & time 
        \\ 
        \shline 
        % GDRNPP & Mask R-CNN~\cite{he2017mask} & RGB & 67.3 & 72.6 & \textbf{83.1} & 58.9 & 34.3 & 82.0 & 80.9 & 68.4 \\
        % GDRNPP & YOLOX~\cite{ge2021yolox} & RGB  & \textbf{71.3} & \textbf{78.6} & \textbf{83.1} & \textbf{62.3} & \textbf{44.8} & \textbf{86.9} & \textbf{82.5} & \textbf{72.8} \\
        % \hline 
        GDRNPP & Mask R-CNN~\cite{he2017mask} & RGB-D  & 77.9  & 83.5  &  \textbf{96.6} & 71.6  & 54.7 & 90.9 & 91.4 & 80.9 \\
        % GDRNPP & YOLOX~\cite{ge2021yolox} & RGB-D & \textbf{80.5} & 89.5 & {96.4} & 73.4 & 68.7 & 94.4 & \textbf{92.9}  & \textbf{85.1} \\
        % \rowcolor{RtwoColorBG} \textbf{GDRNPP}  & YOLOv8~\cite{yolov8} & RGB-D  & 79.4 & \textbf{91.4} & 96.4 & \textbf{73.7} & \textbf{70.4 }& \textbf{95.0} & 92.8 & \textbf{85.6} \\
        \rowcolor{RtwoColorBG} \textbf{GDRNPP}  & YOLOv8~\cite{yolov8} & RGB-D  & \textbf{79.4} & \textbf{91.4} & 96.4 & \textbf{73.7} & \textbf{70.4 }& \textbf{95.0} & \textbf{92.8} & \textbf{85.6} \\
        % \shline 
\end{tabular}
    %\medskip
    %\vspace{-3mm}    
\label{tab:bop_det_model}
\end{table*}


==> gdrn_tables/bop_pe_model.tex <==

\begin{table*}
    \centering
    \tablestyle{8pt}{1.2}
    \small
    \begin{tabular}{l|ccc|ccccccc|c}
        \shline 
        Method & P.E. & Modality & Real
        & LM-O & T-LESS & TUD-L & IC-BIN & ITODD & HB & YCB-V & Avg % & time 
        \\ 
        \hline 
        GDRNPP(ours) & 1 & RGB & \cmark & 68.6 & 77.6 & 82.7 & 61.7 & 26.0 & 80.9 & 76.8 & 67.8 \\
        GDRNPP(ours) & N & RGB & \cmark & 71.3 & 78.6 & 83.1 & 62.3 & 44.8 & 86.9 & 82.5 & 72.8 \\
        \shline 
    \end{tabular}
    \medskip
    \caption{
        {\bf Effect of the number of pose estimator.}
        We report the Average Recall (\%) of the BOP metric.
        P.E. means whether the method is trained with 1 pose estimator for the whole dataset or 1 per object (N objects in total).
    }
\label{tab:bop_pe_model}
\end{table*}


==> gdrn_tables/bop_sota_old.tex <==

\begin{table*}[htbp]
    \centering
    \caption{
        {\bf Comparison with State of the Arts on the BOP core datasets.}
        We report the Average Recall (\%) of the BOP metric.
        The results for other methods are obtained from \href{https://bop.felk.cvut.cz/leaderboards/}{https://bop.felk.cvut.cz/leaderboards/}.
        For each column, we denote the best score in \textbf{bold} and the second best score in \textit{italics}.
        GDRNPP (BOP22) \todo{BOP23 and Ours?} is the BOP Challenge 2022 version of GDRNPP, which utilizes \cite{lipson2022coupled} for depth refinement.
        \Rone{S.M. denotes if the method trains a single model for all objects on each dataset.}
    }
    \begin{threeparttable}[c]
    \tablestyle{6pt}{1.2}
    \small
    \begin{tabular}{l |cc >{\columncolor{RoneColorBG}}c|ccccccc |c | >{\columncolor{RtwoColorBG}}c}
        % \shline 
        Method & Modality & Real & S.M.
        & LM-O & T-LESS & TUD-L & IC-BIN & ITODD & HB & YCB-V & Avg & time(s)
        \\ 
        \shline 
        \textbf{GDRNPP (Ours)} & RGB & \xmark & \xmark & 71.3 & \textbf{79.6} & \textbf{75.2} & \textbf{62.3} & \textbf{44.8} & \textit{86.9} & \textbf{71.3} & \textbf{70.2} & 0.28 \\
        PFA \cite{hu2022perspective} & RGB & \xmark & \cmark & \textbf{74.5} & 71.9 & \textit{73.2} & \textit{60.0} & 35.3 & 84.1 & 64.8 & 66.3 & 3.50 \\
        ZebraPose \cite{su2022zebrapose} & RGB & \xmark & \xmark & \textit{72.1} & 72.3 & 71.7 & 54.5 & \textit{41.0} & \textbf{88.2} & \textit{69.1} & \textit{67.0} & - \\
        SurfEmb \cite{haugaard2022surfemb} & RGB & \xmark & \cmark & 65.6 & \textit{74.1} & 71.5 & 58.5 & 38.7 & 79.3 & 65.3 & 64.7 & 8.89 \\
        EPOS \cite{hodan2020epos} & RGB & \xmark & \cmark & 54.7 & 46.7 & 55.8 & 36.3 & 18.6 & 58.0 & 49.9 & 45.7 & 	1.87 \\
        CDPNv2 \cite{li2019cdpn} & RGB & \xmark & \xmark & 62.4 & 40.7 & 58.8 & 47.3 & 10.2 & 72.2 & 39.0 & 47.2 & 0.98 \\
        DPODv2 \cite{shugurov2021dpodv2} & RGB & \xmark & \xmark & 58.4 & 63.6 & - & - & - & 72.5 & - & - & - \\ 
        CosyPose \cite{labbe2020CosyPose} & RGB & \xmark & \xmark & 63.3 & 64.0 & 68.5 & 58.3 & 21.6 & 65.6 & 57.4 & 57.0 & 0.48 \\ 
        \hline
        \textbf{GDRNPP (Ours)} & RGB & \cmark & \xmark & 71.3 & \textit{78.6} & 83.1 & \textbf{62.3} & \textbf{44.8} & \textit{86.9} & \textit{82.5} & \textbf{72.8} & 0.23 \\
        GDRNPP (S.M.) & RGB & \cmark & \cmark & 68.6 & 77.6 & 82.7 & \textit{61.7} & 26.0 & 80.9 & 76.8 & 67.8 & 0.23  \\
        PFA \cite{hu2022perspective} & RGB & \cmark & \cmark & \textbf{74.5} & 77.8 & \textit{83.9} & 60.0 & 35.3 & 84.1 & 80.6 & 70.9 & 3.02 \\
        ZebraPose \cite{su2022zebrapose} & RGB & \cmark & \xmark & \textit{72.1} & \textbf{80.6} & \textbf{85.0} & 54.5 & \textit{41.0} & \textbf{88.2} & \textbf{83.0} & \textit{72.0} & 0.25 \\
        SurfEmb \cite{haugaard2022surfemb} & RGB & \cmark &  \cmark  & 65.6 & 77.0 & 80.5 & 58.5 & 38.7 & 79.3 & 71.8 & 67.3 & 	8.89 \\
        CRT-6D \cite{castro2023crt} & RGB & \cmark &  \cmark  & 66.0 & 64.4 & 78.9 & 53.7 & 20.8 & 60.3 & 75.2  & 59.9 & 0.06 \\
        Pix2Pose \cite{park2019pix2pose} & RGB & \cmark &  \xmark  & 36.3 & 34.4 & 42.0 & 22.6 & 13.4 & 44.6 & 45.7 & 34.2 & 1.22 \\
        CDPNv2 \cite{li2019cdpn} & RGB & \cmark & \xmark & 62.4 & 47.8 & 77.2 & 47.3 & 10.2 & 72.2 & 53.2 & 52.9 & 	0.94 \\
        %DPODv2 \cite{dpod2} & RGB & \cmark &  & \cmark &  & lmo & 0.655 & tudl & icbin & itodd & hb & ycbv & avg \\ 
        CosyPose \cite{labbe2020CosyPose} & RGB & \cmark & \cmark & 63.3 & 72.8 & 82.3 & 58.3 & 21.6 & 65.6 & 82.1 & 63.7 & 0.45 \\ 
        \hline
        \rowcolor{RtwoColorBG} \textbf{GDRNPP (Ours)} & RGB-D & \xmark & \xmark & 79.4 & \textbf{89.0} & \textit{93.1} & \textbf{73.7} & \textbf{ 70.4} & \textbf{95.0} & 90.1 & \textbf{84.4} & 2.69 \\
        GDRNPP (YOLOX) & RGB-D & \xmark & \xmark & \textbf{80.5} & \textit{88.4} & 92.7 & \textit{73.4} & \textit{68.7} & \textit{94.4} &  \textbf{91.0}  & 84.2 & 4.58 \\
        GDRNPP (BOP22) & RGB-D & \xmark & \xmark & 77.5 & 85.2 & \textit{92.9} & 72.2 & 67.9 & 92.6 & \textit{90.6}  & \textit{82.7} & 6.26 \\
        PFA \cite{hu2022perspective} & RGB-D & \xmark & \cmark &  \textit{79.7} & 80.2 & 89.3 & 67.6 & 46.9 & 86.9 & 82.6 & 76.2 & 2.63 \\
        SurfEmb \cite{haugaard2022surfemb} & RGB-D & \xmark & \cmark & 75.8 & 82.8 & 85.4 & 65.6 & 49.8 & 86.7 & 80.6 & 75.2 & 9.05 \\
        RCVPose3D \cite{wu2022keypoint} & RGB-D & \xmark & \cmark & 72.9 & 70.8 & \textbf{96.6} & 73.3 & 53.6 & 86.3 & 84.3 & 76.8 & 1.34  \\
        Drost \cite{drost2010model} & RGB-D & * & - & 51.5 & 50.0 & 85.1 & 36.8 & 57.0 & 67.1 & 37.5 & 55.0 & 87.57 \\ 
        Vidal Sensors \cite{vidal2018method} & D & * & - & 58.2 & 53.8 & 87.6 & 39.3 & 43.5 & 70.6 & 45.0 & 56.9 & 3.22 \\ 
        \hline
        \rowcolor{RtwoColorBG} \textbf{GDRNPP (Ours)} & RGB-D & \cmark & \xmark & 79.4 & \textbf{91.4} & 96.4 & \textbf{73.7} & \textbf{70.4 }& \textbf{95.0} & \textit{92.8} & \textbf{85.6} & 2.67 \\
        GDRNPP (YOLOX) & RGB-D & \cmark & \xmark & \textbf{80.5} & \textit{89.5} & \textit{96.6} & \textit{73.4} & \textit{68.7} & \textit{94.4} & \textbf{92.9}  & \textit{85.1} & 4.58 \\
        GDRNPP (BOP22) & RGB-D & \cmark & \xmark & 77.5 & 87.4 & \textit{96.6} & 72.2 & 67.9 & 92.6 & 92.1  & 83.7 & 6.26 \\
        PFA \cite{hu2022perspective} & RGB-D & \cmark & \cmark & \textit{79.7} & 85.0 & 96.0 & 67.6 & 46.9 & 86.9 & 88.8 & 78.7 & 2.32 \\
        ZebraPose \cite{su2022zebrapose} & RGB-D & \cmark & \xmark & 75.2 & 72.7 & 94.8 & 65.2 & 52.7 & 88.3 & 86.6 & 76.5 & 0.50 \\
        SurfEmb \cite{haugaard2022surfemb} & RGB-D & \cmark & \cmark & 75.8 & 83.3 & 93.3 & 65.6 & 49.8 & 86.7 & 82.4 & 76.7 & 9.05 \\
        CIR \cite{lipson2022coupled} & RGB-D & \cmark & \cmark & 73.4 & 77.6 & \textbf{96.8} & 67.6 & 38.1 & 75.7 & 89.3 & 74.1 & - \\
        CosyPose \cite{labbe2020CosyPose} & RGB-D & \cmark & \cmark & 71.4 & 70.1 & 93.9 & 64.7 & 31.3 & 71.2 & 86.1 & 69.8 & 13.74 \\ 
        Koenig-Hybrid \cite{konig2020hybrid} & RGB-D & \cmark & \cmark & 63.1 & 65.5 & 92.0 & 43.0 & 48.3 & 65.1 & 70.1 & 63.9 & 0.63 \\
        Pix2Pose \cite{park2019pix2pose} & RGB-D & \cmark & \xmark  & 58.8 & 51.2 & 82.0 & 39.0 & 35.1 & 69.5 & 78.0 & 59.1 &  4.84 \\
        % \shline 
    \end{tabular}
    \medskip
    \begin{tablenotes} 
    \item[] ``Real'' means whether the method uses real-world data for training on T-LESS, TUD-L and YCB-V datasets.
    \item[] ``-'' denotes the results are unavailable and ``*'' denotes the method does not use the provided images for training.
    \end{tablenotes}
\end{threeparttable}
\label{tab:bop_sota}
\end{table*}


==> gdrn_tables/lmo_results_old.tex <==
\begin{table*}
\centering
\tablestyle{5pt}{1.0}
\begin{tabular}{c|c c c c | c c c c | cc}
\shline
\multirow{2}{*}{Method}  & \multicolumn{8}{c|}{w/o Refinement} & \multicolumn{2}{c}{w/ Refinement} \\
\cline{2-11}
 & PoseCNN~\cite{xiang2017posecnn} & PVNet~\cite{peng2019pvnet} & Single-Stage~\cite{hu2020single_stage}  & HybridPose~\cite{song2020hybridpose} & \multicolumn{4}{c|}{GDR-Net (\textbf{Ours})}  & DPOD~\cite{zakharov2019dpod} & DeepIM~\cite{li2019deepim} \\
\hline
P.E. & 1 & $N$ & $N$ & $N$ & 1 & $N$ & 1 & $N$ & 1 & 1 \\
\hline
\tabincell{c}{Training\\Data} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+pbr}} &\tabincell{c}{\texttt{real}\\\texttt{+pbr}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}} & \tabincell{c}{\texttt{real}\\\texttt{+syn}}\\
\hline
Ape	      & 9.6  & 15.8 & 19.2 & 20.9 & 41.3 & 39.3 & 44.9 & 46.8 & - & 59.2 \\
Can		  & 45.2 & 63.3 & 65.1 & 75.3 & 71.1 & 79.2 & 79.7 & 90.8 & - & 63.5 \\
Cat		  & 0.9  & 16.7 & 18.9 & 24.9 & 18.2 & 23.5 & 30.6 & 40.5 & - & 26.2 \\
Driller	  & 41.4 & 65.7 & 69.0 & 70.2 & 54.6 & 71.3 & 67.8 & 82.6 & - & 55.6 \\
Duck      & 19.6 & 25.2 & 25.3 & 27.9 & 41.7 & 44.4 & 40.0 & 46.9 & - & 52.4 \\
Eggbox$^*$& 22.0 & 50.2 & 52.0 & 52.4 & 40.2 & 58.2 & 49.8 & 54.2 & - & 63.0 \\
Glue$^*$  & 38.5 & 49.6 & 51.4 & 53.8 & 59.5 & 49.3 & 73.7 & 75.8 & - & 71.7 \\
Holep.    & 22.1 & 36.1 & 45.6 & 54.2 & 52.6 & 58.7 & 62.7 & 60.1 & - & 52.5 \\
\hline
MEAN	  & 24.9 & 40.8 & 43.3 & 47.5 & 47.4 & \textbf{53.0} & \textbf{56.1} & \textbf{62.2} &47.3&55.5\\
\shline
\end{tabular}
\vspace{-2mm}
\caption{
\label{tab:lmo_sota}
{\bf Comparison with State of the Art on LM-O.}
We report the Average Recall (\%) of ADD(-S). P.E. means whether the method is trained with 1 pose estimator for the whole dataset or 1 per object ($N$ objects in total). ($^*$) denotes symmetric objects and
``-'' denotes unavailable results.
}
\end{table*}


==> gdrn_tables/lmo_ycbv_bop.tex <==
\begin{table*}[t!]
\centering 
\tablestyle{10pt}{1.0}
\begin{tabular}{l | c | c c c | c | c c c | c | c}
\shline
\multirow{2}{*}{Method} &
\multirow{2}{*}{Ref.} &
\multicolumn{4}{c|}{LM-O~\cite{Brachmann2014Learning6O}} &
\multicolumn{4}{c|}{YCB-V~\cite{xiang2017posecnn}} &

\multirow{2}{*}{Time (s)} \\

% \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
\cline{3-10}
& &
$\text{AR}_\text{{\tiny MSPD}}$ &
$\text{AR}_\text{{\tiny MSSD}}$ &
$\text{AR}_\text{{\tiny VSD}}$ &
$\text{AR}$ &
$\text{AR}_\text{{\tiny MSPD}}$ &
$\text{AR}_\text{{\tiny MSSD}}$ &
$\text{AR}_\text{{\tiny VSD}}$ &
$\text{AR}$ & \\

\hline 
AAE~\cite{sundermeyer2018AAE}    &  & 25.4 & 9.5  & 9.0 & 14.6 & 41.0 & 41.3 & 30.7 & 37.7 & 0.190 \\
Pix2Pose~\cite{park2019pix2pose} &  & 55.0 & 30.7 & 23.3 & 36.3 & 57.1 & 42.9 & 37.2 & 45.7 & 1.168 \\
EPOS~\cite{hodan2020epos}        &  & 65.9 & 38.0 & 29.0 & 44.3 & 78.3 & 67.7 & 62.6 & 69.6 & 0.530 \\
CDPNv2~\cite{li2019cdpn} &  & \textit{81.5} & \textit{61.2} & 44.5 & 62.4 & 63.1 & 57.0 & 39.6 & 53.2 & \textit{0.153} \\
GDR-Net (\textbf{Ours}) &  & \textbf{86.4} & \textbf{65.2} & \textbf{50.2} & \textbf{67.2} & \textit{84.2} & \textit{75.6} & \textit{66.8} & \textit{75.5} & \textbf{0.065} \\
\hline
CosyPose~\cite{hodan2020epos} & \checkmark & 81.2 & 60.6 & \textit{48.0} & \textit{63.3} & \textbf{85.0} & \textbf{84.2} & \textbf{77.2} & \textbf{82.1} & 0.395 \\
\shline
\end{tabular}
\caption{\label{tab:lmo_ycb_bop} 
{\bf Results on LM-O and YCB-V under BOP~\cite{hodan_bop20} setup.} 
The results for other methods are obtained from \href{https://bop.felk.cvut.cz/leaderboards/}{https://bop.felk.cvut.cz/leaderboards/}.
The time (s) is the average image processing time averaged over the datasets. Ref. stands for refinement. For each column, we denote the best score in \textbf{bold} and the second best score in \textit{italics}.
} 
\vspace{-0.26em}
\end{table*}


==> gdrn_tables/ycb_results_ADD.tex <==
\begin{table*}[t!]
\centering
\tablestyle{8pt}{1.1}
\begin{tabular}{l | x{80} x{80} x{80} | x{40} x{40}}
% \begin{tabular}{l | c c c | cc }
\shline
Method & PoseCNN~\cite{xiang2017posecnn} & 
% \tabincell{c}{Seg-\\Driven} 
SegDriven~\cite{hu2019segpose} &
% \tabincell{c}{Single-\\Stage} 
Single-Stage~\cite{hu2020single_stage} &
% \tabincell{c}{GDR-Net\\ (\textbf{Ours})} 
\multicolumn{2}{c}{GDR-Net~(\textbf{Ours})} 
\\
\hline
P.E. & 1 & 1 & $N$ & 1 & $N$ \\
\hline 
002\_master\_chef\_can       &  3.6 & 33.0 & -    & 51.7 & 41.5 \\
003\_cracker\_box            & 25.1 & 44.6 & -    & 45.1 & 83.2 \\
004\_sugar\_box              & 40.3 & 75.6 & -    & 83.9 & 91.5 \\
005\_tomato\_soup\_can       & 25.5 & 40.8 & -    & 48.3 & 65.9 \\
006\_mustard\_bottle         & 61.9 & 70.6 & -    & 92.2 & 90.2 \\
007\_tuna\_fish\_can         & 11.4 & 18.1 & -    & 29.1 & 44.2 \\
008\_pudding\_box            & 14.5 & 12.2 & -    & 39.7 & 2.8  \\
009\_gelatin\_box            & 12.1 & 59.4 & -    & 34.6 & 61.7 \\
010\_potted\_meat\_can       & 18.9 & 33.3 & -    & 36.3 & 64.9 \\
011\_banana                  & 30.3 & 16.6 & -    & 60.2 & 64.1 \\
019\_pitcher\_base           & 15.6 & 90.0 & -    & 96.3 & 99.0 \\
021\_bleach\_cleanser        & 21.2 & 70.9 & -    & 73.0 & 73.8 \\
024\_bowl$^*$                & 12.1 & 30.5 & -    & 35.0 & 37.7 \\
025\_mug                     &  5.2 & 40.7 & -    & 39.3 & 61.5 \\
035\_power\_drill            & 29.9 & 63.5 & -    & 57.7 & 78.5 \\
036\_wood\_block$^*$         & 10.7 & 27.7 & -    & 50.8 & 59.5 \\
037\_scissors                &  2.2 & 17.1 & -    & 6.6  & 3.9 \\
040\_large\_marker           &  3.4 &  4.8 & -    & 13.7 & 7.4 \\
051\_large\_clamp$^*$        & 28.5 & 25.6 & -    & 40.3 & 69.8 \\
052\_extra\_large\_clamp$^*$ & 19.6 &  8.8 & -    & 35.3 & 90.0 \\
061\_foam\_brick$^*$         & 54.5 & 34.7 & -    & 61.1 & 71.9 \\
\hline
MEAN                         & 21.3 & 39.0 & 53.9 & 49.1 & \textbf{60.1} \\
\shline
\end{tabular}
% }
\caption{
\label{tab:ycb_results_ADD}
{\bf Detailed results on YCB-V~\cite{xiang2017posecnn} \wrt ADD(-S).}
% Baseline approaches are PoseCNN~\cite{xiang2017posecnn}, SegDriven~\cite{hu2019segpose}, and Single-Stage~\cite{hu2020single_stage}.
P.E. means whether the method is trained with 1 pose estimator for the whole dataset or 1 per object ($N$ objects in total).
($^*$) denotes symmetric objects and ``-'' denotes unavailable results.
}
\end{table*}


==> gdrn_tables/ycb_results_AUC.tex <==
\begin{table*}[t!]
\centering
\tablestyle{4pt}{1.1}
\begin{tabular}{l|cc|c|cc|cc|cc|cc}
\shline
\multirow{2}{*}{Method} & \multicolumn{7}{c|}{w/o Refinement} & \multicolumn{4}{c}{w/ Refinement}\\
\cline{2-12}
 & \multicolumn{2}{c|}{\tabincell{c}{PoseCNN~\cite{xiang2017posecnn}}} & PVNet~\cite{peng2019pvnet} & \multicolumn{4}{c|}{GDR-Net (\textbf{Ours})} & \multicolumn{2}{c|}{\tabincell{c}{DeepIM~\cite{li2019deepim}}} & \multicolumn{2}{c}{\tabincell{c}{CosyPose~\cite{labbe2020CosyPose}}}\\
 \hline
 P.E. & \multicolumn{2}{c|}{1} & $N$ & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{$N$} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c}{1} \\
 \hline 
Metric & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of \\ ADD(-S)}
                  & \tabincell{c}{AUC of\\ADD(-S)}
                  & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of \\ ADD(-S)}
                  & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of \\ ADD(-S)}
                  & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of \\ ADD(-S)}
                  & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of \\ ADD(-S)}\\
\hline
002\_master\_chef\_can       & 84.0 & 50.9 & 81.6 & 96.6 & 71.1 & 96.3 & 65.2 & 93.1 & 71.2 & - & - \\
003\_cracker\_box            & 76.9 & 51.7 & 80.5 & 84.9 & 63.5 & 97.0 & 88.8 & 91.0 & 83.6 & - & - \\
004\_sugar\_box              & 84.3 & 68.6 & 84.9 & 98.3 & 93.2 & 98.9 & 95.0 & 96.2 & 94.1 & - & - \\
005\_tomato\_soup\_can       & 80.9 & 66.0 & 78.2 & 96.1 & 88.9 & 96.5 & 91.9 & 92.4 & 86.1 & - & - \\
006\_mustard\_bottle         & 90.2 & 79.9 & 88.3 & 99.5 & 93.8 & 100.0& 92.8 & 95.1 & 91.5 & - & - \\
007\_tuna\_fish\_can         & 87.9 & 70.4 & 62.2 & 95.1 & 85.1 & 99.4 & 94.2 & 96.1 & 87.7 & - & - \\
008\_pudding\_box            & 79.0 & 62.9 & 85.2 & 94.8 & 86.5 & 64.6 & 44.7 & 90.7 & 82.7 & - & - \\
009\_gelatin\_box            & 87.1 & 75.2 & 88.7 & 95.3 & 88.5 & 97.1 & 92.5 & 94.3 & 91.9 & - & - \\
010\_potted\_meat\_can       & 78.5 & 59.6 & 65.1 & 82.9 & 72.9 & 86.0 & 80.2 & 86.4 & 76.2 & - & - \\
011\_banana                  & 85.9 & 72.3 & 51.8 & 96.0 & 85.2 & 96.3 & 85.8 & 91.3 & 81.2 & - & - \\
019\_pitcher\_base           & 76.8 & 52.5 & 91.2 & 98.8 & 94.3 & 99.9 & 98.5 & 94.6 & 90.1 & - & - \\
021\_bleach\_cleanser        & 71.9 & 50.5 & 74.8 & 94.4 & 80.5 & 94.2 & 84.3 & 90.3 & 81.2 & - & - \\
024\_bowl$^*$                & 69.7 & 69.7 & 89.0 & 84.0 & 84.0 & 85.7 & 85.7 & 81.4 & 81.4 & - & - \\
025\_mug                     & 78.0 & 57.7 & 81.5 & 96.9 & 87.6 & 99.6 & 94.0 & 91.3 & 81.4 & - & - \\
035\_power\_drill            & 72.8 & 55.1 & 83.4 & 91.9 & 78.7 & 97.5 & 90.1 & 92.3 & 85.5 & - & - \\
036\_wood\_block$^*$         & 65.8 & 65.8 & 71.5 & 77.3 & 77.3 & 82.5 & 82.5 & 81.9 & 81.9 & - & - \\
037\_scissors                & 56.2 & 35.8 & 54.8 & 68.4 & 43.7 & 63.8 & 49.5 & 75.4 & 60.9 & - & - \\
040\_large\_marker           & 71.4 & 58.0 & 35.8 & 87.4 & 76.2 & 88.0 & 76.1 & 86.2 & 75.6 & - & - \\
051\_large\_clamp$^*$        & 49.9 & 49.9 & 66.3 & 69.3 & 69.3 & 89.3 & 89.3 & 74.3 & 74.3 & - & - \\
052\_extra\_large\_clamp$^*$ & 47.0 & 47.0 & 53.9 & 73.6 & 73.6 & 93.5 & 93.5 & 73.3 & 73.3 & - & - \\
061\_foam\_brick$^*$         & 87.8 & 87.8 & 80.6 & 90.4 & 90.4 & 96.9 & 96.9 & 81.9 & 81.9 & - & - \\
\hline
MEAN                         & 75.9 & 61.3 & 73.4 & 89.1 & 80.2 & \textbf{91.6} & \textbf{84.3} & 88.1 & 81.9 & 89.8 & \textbf{84.5} \\
\shline
\end{tabular}
\caption{
\label{tab:ycb_results_AUC}
{\bf Detailed results on YCB-V~\cite{xiang2017posecnn} \wrt AUC of ADD-S and ADD(-S).}
As in \cite{xiang2017posecnn}, ADD-S uses the symmetric metric for all objects, while ADD(-S) only uses the symmetric metric for symmetric objects.
P.E. means whether the method is trained with 1 pose estimator for the whole dataset or 1 per object ($N$ objects in total).
($^*$) denotes symmetric objects and ``-'' denotes unavailable results.
}
\end{table*}


==> gdrn_tables/ycb_results_simple.tex <==

\begin{table}
\centering
\tablestyle{5pt}{1.0}
\begin{tabular}{c|c|c|ccc}
\shline
Method                                & Ref. & P.E.& ADD(-S)  & \tabincell{c}{AUC of\\ADD-S} & \tabincell{c}{AUC of\\ADD(-S)}  \\
\hline
PoseCNN~\cite{xiang2017posecnn}       &      & 1   & 21.3     & 75.9       & 61.3 \\
SegDriven~\cite{hu2019segpose}        &      & 1   & 39.0     & -          &  -   \\
PVNet~\cite{peng2019pvnet}            &      & $N$ & -        & -          & 73.4 \\
Single-Stage~\cite{hu2020single_stage}&      & $N$ & 53.9     & -          & -    \\
\hline 
GDR-Net (\textbf{Ours})               &      & $1$ & 49.1     & 89.1       & 80.2 \\
GDR-Net (\textbf{Ours})               &      & $N$ &{\bf 60.1}& {\bf 91.6} & 84.4 \\
\hline
DeepIM~\cite{li2019deepim}            & \checkmark & 1 & -        & 88.1       & 81.9 \\
CosyPose~\cite{labbe2020CosyPose}     & \checkmark & 1 &  -       & 89.8       & {\bf 84.5} \\
\shline
\end{tabular}

\vspace{-2mm}
\caption{
\label{tab:ycb_simple}
{\bf Comparison with State of the Art on YCB-V.}
We report the results evaluated \wrt ADD(-S), and AUC of ADD-S and ADD(-S). 
As in \cite{xiang2017posecnn}, ADD-S uses the symmetric metric for all objects, while ADD(-S) only uses the symmetric metric for symmetric objects.
P.E. means whether the method is trained with 1 pose estimator for the whole dataset or 1 per object ($N$ objects in total).
Ref. stands for Refinement and
``-'' denotes unavailable results.}
\end{table}

